Production of light-flavor hadrons in pp collisions at $\sqrt{s}$ = 7 and $\sqrt{s}$ = 13 TeV

The production of $\pi^{\pm}$, $\rm{K}^{\pm}$, $\rm{K}^{0}_{S}$, $\rm{K}^{*}(892)^{0}$, $\rm{p}$, $\phi(1020)$, $\Lambda$, $\Xi^{-}$, $\Omega^{-}$, and their antiparticles was measured in inelastic proton-proton (pp) collisions at a center-of-mass energy of $\sqrt{s}$ = 13 TeV at midrapidity ($|y|<0.5$) as a function of transverse momentum ($p_{\rm{T}}$) using the ALICE detector at the CERN LHC. Furthermore, the single-particle $p_{\rm{T}}$ distributions of $\rm{K}^{0}_{S}$, $\Lambda$, and $\overline{\Lambda}$ in inelastic pp collisions at $\sqrt{s}$ = 7 TeV are reported here for the first time. The $p_{\rm{T}}$ distributions are studied at midrapidity within the transverse momentum range $0\leq p_{\rm{T}}\leq20$ GeV/$c$, depending on the particle species. The $p_{\rm{T}}$ spectra, integrated yields, and particle yield ratios are discussed as a function of collision energy and compared with measurements at lower $\sqrt{s}$ and with results from various general-purpose QCD-inspired Monte Carlo models. A hardening of the spectra at high $p_{\rm{T}}$ with increasing collision energy is observed, which is similar for all particle species under study. The transverse mass and $x_{\rm{T}}\equiv2p_{\rm{T}}/\sqrt{s}$ scaling properties of hadron production are also studied. As the collision energy increases from $\sqrt{s}$ = 7 to 13 TeV, the yields of non- and single-strange hadrons normalized to the pion yields remain approximately constant as a function of $\sqrt{s}$, while ratios for multi-strange hadrons indicate enhancements. The $p_{\rm{T}}$-differential cross sections of $\pi^{\pm}$, $\rm{K}^{\pm}$ and $\rm{p}$ ($\overline{\rm{p}}$) are compared with next-to-leading order perturbative QCD calculations, which are found to overestimate the cross sections for $\pi^{\pm}$ and $\rm{p}$ ($\overline{\rm{p}}$) at high $p_{\rm{T}}$.

==> c <==
#!/bin/bash

if [ -z "$1" ];then
echo -en "\n\n\tUsage: $0 /path/to/TeX/file\n\n"
echo -en "\tExample: ./c ./alicepreprint_CDS.tex\n\n"
exit 99;
fi

filename=$(basename $1)
extension=${filename##*.}
filename=${filename%.*}

PWD=`pwd`
LOG="${PWD}/compile.log"

rm -vf *.{aux,dvi,log,spl,ps,bbl,blg}

clear;
echo -en "\n\n\tCompiling LaTeX document $1 at `date +"%r"`...\n" &&
pdflatex -shell-escape $1 > /dev/null && 
echo -en "\n\t\tx 1 times ...\t\t\t\t[ OK ]\n" &&

bibtex $filename &&

pdflatex -shell-escape $1 > /dev/null && 
echo -en "\t\tx 2 times ...\t\t\t\t[ OK ]\n" &&

pdflatex -shell-escape $1 > /dev/null && 
echo -en "\t\tx 3 times ...\t\t\t\t[ OK ]\n\n" &&
echo -en "Opening $filename.pdf ...\t\t\t\t[ OK ]\n" &&

############acroread $filename.pdf 2>/dev/null&
acroread $filename.pdf 2>/dev/null&

